ProxyDet: Synthesizing Proxy Novel Classes via Classwise Mixup for Open-Vocabulary Object Detection

Open-vocabulary object detection (OVOD) aims to recognize novel objects whose categories are not included in the training set. In order to classify these unseen classes during training, many OVOD frameworks leverage the zero-shot capability of largely pretrained vision and language models, such as CLIP. To further improve generalization on the unseen novel classes, several approaches proposed to additionally train with pseudo region labeling on the external data sources that contain a substantial number of novel category labels beyond the existing training data. Albeit its simplicity, these pseudo-labeling methods still exhibit limited improvement with regard to the truly unseen novel classes that were not pseudo-labeled. In this paper, we present a novel, yet simple technique that helps generalization on the overall distribution of novel classes. Inspired by our observation that numerous novel classes reside within the convex hull constructed by the base (seen) classes in the CLIP embedding space, we propose to synthesize proxy-novel classes approximating novel classes via linear mixup between a pair of base classes. By training our detector with these synthetic proxy-novel classes, we effectively explore the embedding space of novel classes. The experimental results on various OVOD benchmarks such as LVIS and COCO demonstrate superior performance on novel classes compared to the other state-of-the-art methods. Code is available at https://github.com/clovaai/ProxyDet.

==> figures/table1_figure2_mixed.tex <==
\begin{figure*}
    \begin{minipage}[t]{.48\linewidth}
        %--------------------------------------------------------------------------
            \centering
            \includegraphics[width=1\textwidth]{figures/analyze_mixup_sim_novel_LVIS novel_top1_plot}
                \label{fig:novel_similarity_distribution}
            \caption{\textbf{Similarity of mixed classes with novel classes.} We use base classes defined in LVIS dataset and mix CLIP~\cite{clip} text embeddings of these base classes. For visualizing (a), novel classes are sorted with ascending order by similarity b.t.w. base classes.
            Similarity distribution for top-1 cosine similarity b.t.w. each of novel class and all the mixed (or base) classes.
            % Newly mixed proxy embeddings can better represent novel classes.
            % Newly mixed embeddings can better represent novel classes defined on (a) (LVIS \cite{gupta2019lvis} dataset) and (b) (the more real-world case \cite{ridnik2021imagenet} where base and novel distribution is distinct and size of novel set is large (21K)).
            }
            \label{fig:novel_similarity}
        % \end{figure}
        %------------------------------------
    \end{minipage}
    \hfill
  \begin{minipage}[b]{0.48\linewidth}
        % \begin{table}[t]
        
        \centering
        \smallskip\noindent
        \tabcolsep=0.1cm
        \resizebox{1\linewidth}{!}{
        \begin{tabular}{cc|ccc}
        \toprule
        
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Pseudo-labeling? \end{tabular}} & 
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Ours \end{tabular}} & 
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Ovl $AP_r$
        \end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Non-ovl $AP_r$\end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Overall $AP_r$ \end{tabular}} \\ 
        & & &   \\
        \midrule
        
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red2}{\ding{56}}  \end{tabular}} & 
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red2}{\ding{56}}  \end{tabular}} & 
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} 15.8 \\ (+0.0)
        \end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} 20.2 \\ (+0.0) \end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} 16.7 \\ (+0.0) \end{tabular}} \\ 
        & & &   \\
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red2}{\ding{56}}  \end{tabular}} & 
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{darkergreen}{\ding{52}}  \end{tabular}} & 
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} -	\\ 
        \end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} - \\  \end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} 18.9 \\ \textbf{\textcolor{red2}{(+2.2)}} \end{tabular}} \\ 
        & & &   \\
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  \textcolor{darkergreen}{\ding{52}}  \end{tabular}} & 
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red2}{\ding{56}} \end{tabular}} & 
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} 25.7 \\ \textcolor{darkergreen}{(+9.9)}
        \end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} 21.5 \\ \textcolor{darkergreen}{(+1.3)} \end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} 24.9 \\ \textcolor{darkergreen}{(+8.2)} \end{tabular}} \\ 
        & & &   \\
        
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  \textcolor{darkergreen}{\ding{52}}\end{tabular}} & 
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}   \textcolor{darkergreen}{\ding{52}}\end{tabular}} & 
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} 27.0 \\ \textbf{\textcolor{darkergreen}{(+11.2)}}
        \end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} 23.6 \\ \textbf{\textcolor{red2}{(+3.4)}} \end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} 26.3 \\ \textbf{\textcolor{darkergreen}{(+9.6)}} \end{tabular}} \\ 
        & & &   \\
        \bottomrule
        
        \end{tabular}
        }
        \caption{\textbf{Effect of pseudo-labeling \cite{detic} and ProxyDet (ours) on the generalization performance towards unseen classes.} Ovl $AP_r$ / Non-ovl $AP_r$: performance of novel classes divided by whether used for pseudo-labeling or not.
        Notably, pseudo-labeling results in marginal performance improvement concerning genuinely novel classes (i.e., non-overlapping ones). However, our ProxyDet strategy significantly enhances the performance.
        }
        \label{table:table1_nonovl_ap}
        % \end{table}
  \end{minipage}
\end{figure*}

==> manuscripts/3_methods_before.tex <==
%\input{figures/overview}
\section{Method}

We briefly review the overall framework of OVOD methods with notation clarification. Then, we present our ProxyDet which trains with proxy novel classes to enhance the classification ability on novel classes without the prior knowledge (\hskim{(i.e., names)} of the novel classes.

% method 세부 섹션
% 3.1 - Overview
% Vanilla OVD (VilD Text, zeroshot clip의 활용)
%     1. Traidiontal closed-set object detector 세팅 formulation & open-set obect detector formulation 설명
%     2. mixup 알고리즘 figure 설명. 간단한 설명 및 목적. 그리고 Section 3.2, 3.3에서 어떤것을 다룰것인지? 에 대한 설명.

\subsection{Notations and Preliminaries}
\label{method:overview_3_1}
Object detector is trained on a dataset $D = \{(I_i, g_i)\}_{i=1}^{|D|}$ where $I_i$ refers to $i$-th image and $g_i = \{(b_k, c_k)\}_{k=1}^{K}$ denotes object bounding boxes ($b_k$) and corresponding class labels ($c_k \in \mathcal{C}_{\text{B}} $) where $\mathcal{C}_{\text{B}}$ is the set of base classes. Open-Vocabulary Object Detection (OVOD) aims to detect not only the base classes $\mathcal{C}_{\text{B}}$ but also novel classes $\mathcal{C}_{\text{N}}$ where $\mathcal{C}_{\text{B}} \cap \mathcal{C}_{\text{N}} = \emptyset$. 
In OVOD training, given batch of images $\{I_1,\cdots,I_n\}$, Regional Proposal Network (RPN)\cite{centernet2} generates a set of regional proposals $\bm{P}$ for images and positive proposals $\bm{p}$ ($\bm{p}_{+} \subset \bm{P}$) with high IoUs with ground-truth bounding boxes for base class are selected. Each of positive proposal $p \in \bm{p}$ is vectorized into region embedding $\bm{r} \in \mathbb{R^{M}}$ using detector head with ROI-Align~\cite{mask_rcnn} where . Cross-Entropy~(CE) loss is applied using cosine similarity between the regional embeddings and text embeddings of base classes cached from a pre-trained text encoder $\mathcal{T}(\cdot)$ such as CLIP. 
%ViLD~\cite{vild} utilizes knowledge distillation to align the latent space of the object detector with that of CLIP to obtain representations of novel classes without any previous exposure to their visual or textual information.

%To obtain the representations of novel categories without prior exposure to their visual or textual information, ViLD~\cite{vild} utilize knowledge distillation to match image embedding space 
%pre-trained image encoder to match 
%%

%CLIP 들어가야함. 



%re selected whose IoUs with respect to one ground-truth bounding box $b \in \mathcal{C}_{\text{B}} $ are higher than a threshold. The positive proposals are then vectorized into one dimensional embedding $\bm{r} \in \mathbb{R^{M}}$ through detector head with ROI-Align~\cite{mask_rcnn} and cascade classification layers~\cite{cascade_rcnn}. For classification training w.r.t. base class objects, we applied cross entropy (CE) loss using cosine similarity b.t.w. regional embeddings and text embeddings of base class $\mathcal{T}(\mathcal{C}_{\text{B}})$ as in~\cite{vild}

%  \paragraph{Notations and Preliminaries} For training, given batch of images $\{I_{1,...,n}\}$, we obtain a set of proposals $\bm{p}$ for the overall images via regional proposal network (RPN)~\cite{centernet2}. Among the overall proposals, we obtain positive proposals $\bm{p_{\text{pos}}}$ whose IoUs w.r.t. one ground-truth bounding box $b \in \mathcal{C}_{\text{B}} $ are higher than a threshold (i.e. 0.5).
 %Since RPN is pre-trained on base classes as in \cite{detic}, RPN proposals can partially or fully localize base class objects.
 
 %The positive proposals are then vectorized into one dimensional embedding $\bm{r} \in \mathbb{R^{M}}$ through detector head with ROI-Align~\cite{mask_rcnn} and cascade classification layers~\cite{cascade_rcnn}. For classification training w.r.t. base class objects, we applied cross entropy (CE) loss using cosine similarity b.t.w. regional embeddings and text embeddings of base class $\mathcal{T}(\mathcal{C}_{\text{B}})$ as in~\cite{vild}.



%Several works \cite{} utilize additional unlabeled datasets and vocabulary of novel classes $\mathcal{C}_{\text{B}}$  to learn the representations of novel classes. However, the performance on test dataset of non-overlapped novel classes are limited. To this end, 
%To enhance the classification ability on novel classes even without the prior knowledge of novel classes, we propose the learning strategy which train an OVOD model with proxy-novel classes which generated via class-wise mixup between representations of base classes. Overall framework of ProxyDet is illustrated in Fig \ref{fig:overview}. 
%In the subsequent section, we describe how to synthesize proxy-novel class representations in Section \ref{method:learning_proxy_novel_classes_3_2}.
% In the subsequent sections, we firstly describe how to synthesize proxy-novel class representations in Section \ref{method:learning_proxy_novel_classes_3_2}, followed by the enhanced methodologies for more robust and better novel class approximation in Section \ref{method:towards_better_robustness_and_novel_approximation_3_3}.

\subsection{ProxyDet: Learning Proxy Novel Classes via Class-wise Mixup}
\label{method:learning_proxy_novel_classes_3_2}
%%% ...notation 정리 필요
% 3.2. LEARNING PROXY-NOVEL class representations BY CLASS-WISE Mixup
%     1. mixup 
%         1. 어떻게 mixup하는거고 (formulation. base class cross entropy설명 필요.)
%         2. architecure flow 더 자세히 설명
%         3. algorithm 설명 (simple하다)
%         4. test-time fusion 설명

To facilitate the model's ability to recognize new categories during test phase, it is crucial to expand the boundary of the visual and textual representations towards novel classes. To achieve this, we generate the proxy-novel by separately combining the visual and textual class prototypes belonging to seen classes, and then regulate them close each other. 

%the visual~$r_{\text{novel}} \in \mathcal{C}_{\text{N}}$ and textual $r_{\text{novel}}$ representations towards novel classes. 
%To achieve this, we generate the proxy-novel by separately combining the visual and textual class prototypes belonging to seen classes. 
%based solely on existing knowledge, 
%we generate the proxy-novel by separately combining the visual and textual class prototypes belonging to seen classes. 
%Here, we aim to train a detector on large set of proxy-novel classes for generalization on true novel classes. To achieve this goal, we devise a class-wise mixup technique that linearly interpolates representation of base classes to synthesize that of proxy-novel classes.

%Visual and Textual Prototype.
\paragraph{Synthesizing Proxy-Novel.} 
Textual embeddings can be matched one-to-one with their respective base classes. However, this is not the case for visual embeddings, where each base class is associated with multiple region proposals. Therefore, we establish visual class prototypes as the initial step in our approach. Consider a set of region embeddings from RPN and corresponding class~$\{(r_i, c_i)\}_{i=1}^P$ where $P$ is the number of extracted positive proposals in a batch. A simple and naive approach is to construct a visual prototype embedding by averaging the regional embeddings that belong to the class as formulated below. 

\begin{equation}
\begin{split}
    & P_{\text{c}} = \big\| \sum_{i \in {c}} F(\bm{r}) * r_i \big\|_{2} \\
    \text{where} \quad & F(\bm{r}) = \frac{1}{|c_i = c \in \{(r_i, c_i)\}_{i=1}^P|}
    \label{eq:prototype}
\end{split}
\end{equation}

 \paragraph{Proxy Loss.} For a regional embedding of novel class $r_{\text{novel}} \in \mathcal{C}_{\text{N}}$ to be accurately classified during test phase, it is essential for $r_{\text{novel}}$ to be close to the text embedding of novel class. Therefore, we approximately regularize the proximal regional embedding of $r_{\text{novel}}$, namely $r_{\text{proxy}}$, to minimize its distance with the proxy-novel text embedding $\mathcal{T}(\mathcal{C}_{\text{proxy}})$ where $\mathcal{T}(\cdot)$ denotes pre-trained text encoder of CLIP.
% 위 목적을 달성하기 위하여, $r^{proxy}~= r^{novel}$이 proxy-novel text embedding $T~\mathcal{C}_{\text{N}}$ (which is approximately novel as show in figure 2)에 가까워지도록 학습할 수 있도록 한다. 
Our objective can be formulated as follows:

\begin{equation}
    \mathcal{L}_{proxy} = \frac{1}{S} \sum_{c \sim P_{\text{proxy}}} || \mathcal{T}(\mathcal{C}_\text{c}) - r_{\text{c}} ||_{1}
\label{eq:proxy_loss}
\end{equation}

where $S$ denotes number of sampling from proxy-novel distribution $P_{proxy}$. To synthesize representations of proxy-novel classes, we apply class-wise mixup b.t.w. embedding of base classes, based on the observations from Figure \ref{fig:novel_similarity}:
\begin{equation}
\begin{split}
    & \mathcal{T}(\mathcal{C}_{\text{proxy}}) = ||\ \lambda \mathcal{T}(\mathcal{C}_{\text{B}_{i}}) + (1 - \lambda) \mathcal{T}(\mathcal{C}_{\text{B}_{j}})\ ||_{2} \\
    & r_{\text{proxy}} = ||\ \lambda r_{\text{B}_{i}} + (1 - \lambda) r_{\text{B}_{j}}\ ||_{2}
\end{split}
\label{eq:mixup}
\end{equation}

where $\lambda \sim Beta(\gamma, \gamma)$ and $B_i, B_j$ are random-uniformly sampled from one of base classes appeared within image batch. Notably, although class-specific text embeddings $\mathcal{T}(\mathcal{C}_{\text{B}_{i, j}})$ can be easily obtained by forwarding through largely pretrained text encoder of VL models, acquiring class-specific regional embedding $r_{\text{B}_{i, j}}$ is non-trivial since there are a number of candidate regional embeddings that can represent class $B_{i}$ or $B_{j}$. A simple and naive approach is to construct a prototype embedding that is capable of representing a particular base class by averaging the regional embeddings that belong to the class:

\begin{equation}
\begin{split}
    r_{\text{B}_{i}} = || \sum_{r \sim \bm{r}_{\text{B}_{i}}} F(r) * r\ ||_{2}
\end{split}
\label{eq:prototype}
\end{equation}

 where $\bm{r}_{\text{B}_{i}}$ refers to a subset of positive proposals that are matched with objects that have class label $\text{B}_{i}$, and $F(r) = \frac{1}{|\bm{r}_{\text{B}_{i}}|}$.

% RPN에서 나온 proposal들을 class별로 groupping한다. (by IoU Thresholding) 
% base class를 대표할 수 있는 prototype을 만든다.
 % base prorotype들을 활용하여 proxy novel prototyep 을 만들고, 이게 proxy-novel text embedding에 가까워지도록 mixup을 통해 학습하도록 한다.
 % mixup formulation. batch내에 있는 모든 class들에 대해서 class-wise mixup. pair결정은 random으로 표기. (equation 하나 나와야할듯.)

% class를 대표할 수 있는 prototype embedding 구해서,
% mixup(prototype embedding of class a, prototype embedding of class b)이 mixup(text embedding of class a, text embedding of class b)에 따라가게끔 학습한다. 

\paragraph{Robust Prototype.} Simply averaging all the regional embeddings for constructing a prototype embedding as in Eq (\ref{eq:prototype}) can be sub-optimal since the visual semantics and contexts of the proposals that belong to the same class vary (Figure \ref{fig:prototype}). To cope with this, we propose to construct a robust prototype tailored to better represent the class specific features by modulating the weighting function $F(r)$ with proposal quality-aware measure $L$:

\begin{equation}
\begin{split}
    F(r) = \frac{\text{exp}(L(r))}{\sum_{\tilde{r} \sim \bm{r}_{\text{B}_{i}}} \text{exp}( L(\tilde{r}))}
\end{split}
\label{eq:prototype_weighting_function}
\end{equation}

Notably, $L$ can be defined by \textit{objectness score} from RPN or \textit{IoU} with matched ground-truth box. Through Eq (\ref{eq:prototype_weighting_function}), our proxy-novel synthesis (Eq (\ref{eq:mixup})) is conditioned on more robust prototype embeddings that can better estimate the base class representations.

\input{figures/prototype}

% As the positive proposals contain different visual contexts as shown in Figure \ref{}, we propose to construct a robust prototype tailored for better representing the class-specific features. 

% Therefore, Simply averaging all the regional embeddings $r \sim \bm{r}_{\text{B}_i}$ for constructing prototype embedding might induce 

% For constructing the prototype of embedding $$, 

%         1. instance-wise mixup은 기존에 있었다. 그러나, ~~이유로 robust한 prototype embedding을 못만들고 , mixup할때 sub-optimal일수있다.
%         2. 따라서, 우리는 좀 더 robust한 prototype을 가지고 class-wise mixup를 제안한다. 
%         3. 그러나, quality가 좋지 않은 embedding들이 prototype에 참여되면, 이또한 potential caveat이다.
%         4. 따라서, objectness score나 iou를 기반으로 좋은 quality proposal embedding만 가지고 prototype embedding을 만들어 내겠다.

 \paragraph{Separated Head.} Since our proxy loss Eq (\ref{eq:proxy_loss}) aims to enhance novel classification while conventional CE loss focuses on that of base classes, we applied each of loss separately on two separated detector heads with identical architecture~\cite{vild, f-vlm}. 
 For inference, we combine both of classification scores from two heads by geometric mean, following~\cite{f-vlm}:

\begin{equation}
    s_i = 
\begin{cases}
    (r' w^{\top})^{1-\alpha}_{i} *  (r w^{\top})^{\alpha}_{i}, & \text{if } i \in \mathcal{C}_{\text{B}} \\
    (r' w^{\top})^{1-\beta}_{i} *  (r w^{\top})^{\beta}_{i}, & \text{if } i \in \mathcal{C}_{\text{N}}
\end{cases}
\label{eq:score_fusion}
\end{equation}

where $w = \mathcal{T}(\mathcal{C}_{\text{B}} \cup \mathcal{C}_{\text{N}})$, $\ s_i$ is final classification score for $i$-th class and $r$ and $r'$ are regional embeddings from a head trained with proxy loss and the other head with CE loss, respectively.  $\alpha, \beta \in [0, 1]$ determines the ratio of reflecting classification scores from proxy loss head for base/novel categories.
 % classification loss랑 mixup loss랑 contention이 있어서,  똑같은 roi head 구조를 2개 둬서, 서로 다른 supervision이 들어가도록 했다.

 % \paragraph{Inference}
 % inference할때는 geometric mean해줬다 (f-vlm) 
 
% 왜 novel class에 대해 잘 동작할 수 있는가? 1번 이유) 실제로 novel class에 대한 proposal이 조금 더 proxy-novel space에 가까워지도록 되게 되서 (which is approximately novel as show in figure 2), 더 novel class에 대한 classification을 잘할 수 있게 된다.
% 왜 novel class에 대해 잘 동작할 수 있는가? 2번 이유) detector가 l1으로 proxy class text embedding에 유사해지도록 학습되면, 실제 novel class object가 들어왔을때, 이를 novel class text embedding에 유사해지도록 할 수 있을것이다. 따라서, novel class에 대해서 더욱 classification을 잘할 수 있게 된다.
% dense하게 한다. 그래서 최대한 많은 novel class들을 approximate되게끔한다.

% \subsection{Towards better robustness and novel class approximation}
% \label{method:towards_better_robustness_and_novel_approximation_3_3}
% \paragraph{Robust Prototype} For constructing the class-specific regional embeddings, we simply averaged regional embeddings of a class   leverage Instead of instance-wise mixup, 

% 3.3. TOWARDS better robustness and novel class approximation
%     1. mixup granularity
%         1. instance-wise mixup은 기존에 있었다. 그러나, ~~이유로 robust한 prototype embedding을 못만들고 , mixup할때 sub-optimal일수있다.
%         2. 따라서, 우리는 좀 더 robust한 prototype을 가지고 class-wise mixup를 제안한다. 
%         3. 그러나, quality가 좋지 않은 embedding들이 prototype에 참여되면, 이또한 potential caveat이다.
%         4. 따라서, objectness score나 iou를 기반으로 좋은 quality proposal embedding만 가지고 prototype embedding을 만들어 내겠다.
%     2. mixup class pair.
%             1. random하게 class를 섞는 방법
%             2. novel class pairing: novel class를 조금 더 근사해보기 위해서, ideal case를 해본다. (using intractable knowledge: novel category space)
%     3. distill과의 비교? (optional)
%         1. 어떤점에서 distill과 차별성이 있는지 짚어주기. 의미론적으로.
%             1. text embedindg 직접 맞춰준다 (which has similar semantics with novel classes)
%             2. training time때 offline proposal들을 뽑는 공수가 안든

% \begin{enumerate}
%     \item \todo{ identified the limitations of existing approaches}
%     \item \todo{ I am tackling existing solutions limitations.}
%     \item \todo{ giving an overview of my approach, telling how it works in a general way. (explained your approach in general terms)}
%     \item \todo{ motivated your solution using Figure: show a picture of how your approach will deal with such a problem. }
% \end{enumerate}




% method notation 정리 안된 버전 (detail한 수식들 기반; 가독성 떨어짐)

% \input{figures/overview}
% \section{Method (Joonhyun)}

% We briefly review the overall framework of OVOD methods with notation clarification. Then, we present our ProxyDet (Figure \ref{fig:overview}) which trains with proxy novel classes to enhance the classification ability on novel classes without the prior knowledge of the novel classes.

% % method 세부 섹션
% % 3.1 - Overview
% % Vanilla OVD (VilD Text, zeroshot clip의 활용)
% %     1. Traidiontal closed-set object detector 세팅 formulation & open-set obect detector formulation 설명
% %     2. mixup 알고리즘 figure 설명. 간단한 설명 및 목적. 그리고 Section 3.2, 3.3에서 어떤것을 다룰것인지? 에 대한 설명.

% \subsection{Notations and Preliminaries}
% \label{method:overview_3_1}
% An object detector is trained on a dataset $D = \{(I_i, g_i)\}_{i=1}^{|D|}$ where $I_i$ refers to an $i$-th image and $g_i = \{(b^{gt}_k, c_k)\}_{k=1}^{|g_i|}$ denotes a set of ground-truth object labels consisting of a bounding box ($b^{gt}_k$) and the corresponding class label ($c_k \in \mathcal{C}^{\text{B}} $) where $\mathcal{C}^{\text{B}}$ is the entire set of base classes. At the inference phase, Open-Vocabulary Object Detection (OVOD) aims to detect not only the base classes $\mathcal{C}^{\text{B}}$ but also novel classes $\mathcal{C}^{\text{N}}$ which satisfy $\mathcal{C}^{\text{B}} \cap \mathcal{C}^{\text{N}} = \emptyset$. 

% In OVOD training, given batch of images $I = \{I_i\}_{i=1}^{n}$, Regional Proposal Network (RPN)\cite{centernet2} generates a set of regional proposals $p_i$ for all the images $I$:
% \begin{equation}
%     p_{ij} = \{(b^{p}_{ij}, o_{ij}, u_{ij}, c_{ij})\}_{j=1}^{|\bm{p_i}|}
% \label{eq:proposal_def}
% \end{equation}

% where $|p_i|$ denotes the number of proposals predicted on $I_i$ and $b^{p}_l, o_l, u_l, c_l$ denote box location, predicted objectness score, IoU with the nearest ground-truth bounding box $\tilde{b}^{gt}$, and assigned class label $c_l$ that corresponds to the class label of $\tilde{b}^{gt}$, respectively.


% A set of positive proposals in the batch is aggregated by concatenating each positive subset of $\bm{p_i}$, $\bm{p^{pos}} = (\bm{p_{1}^{pos}} \cup \bm{p_{2}^{pos}} \cdots \cup \ \bm{p_{n}^{pos}})$ where $\bm{p_i^{pos}}$ refers to a set of proposals whose IoU with ground-truth box ($u$) is higher than a threshold (e.g. 0.5).
% % Among $\bm{p}$, positive proposals $\bm{p_{\text{pos}}} = $ with high IoUs with ground-truth bounding boxes for base classes are selected. 
% Each of positive proposal $p^{pos} \in \bm{p^{pos}}$ is then vectorized into one-dimensional regional embedding $r^{pos} \in \mathbb{R^{M}}$ through a detector head $R(\cdot)$ with ROI-Align~\cite{mask_rcnn} and a few fully-connected layers:
% \begin{equation}
%     r^{pos} = \mathcal{R}(p^{pos})
% \label{eq:detector_head}
% \end{equation}

% For classification training with regard to the base class objects, Cross-Entropy~(CE) loss is applied using cosine similarity between the positive regional embedding $r^{pos}$ and text embeddings of base classes $\mathcal{T}(\mathcal{C}^{\text{B}})$ from a pre-trained text encoder $\mathcal{T}(\cdot)$ such as CLIP.
% % ViLD~\cite{vild} utilizes knowledge distillation to align the latent space of the object detector with that of CLIP to obtain representations of novel classes without any previous exposure to their visual or textual information.

% %To obtain the representations of novel categories without prior exposure to their visual or textual information, ViLD~\cite{vild} utilize knowledge distillation to match image embedding space 
% %pre-trained image encoder to match 
% %%

% %CLIP 들어가야함. 



% %re selected whose IoUs with respect to one ground-truth bounding box $b \in \mathcal{C}^{\text{B}} $ are higher than a threshold. The positive proposals are then vectorized into one dimensional embedding $\bm{r} \in \mathbb{R^{M}}$ through detector head with ROI-Align~\cite{mask_rcnn} and cascade classification layers~\cite{cascade_rcnn}. For classification training w.r.t. base class objects, we applied cross entropy (CE) loss using cosine similarity b.t.w. regional embeddings and text embeddings of base class $\mathcal{T}(\mathcal{C}^{\text{B}})$ as in~\cite{vild}

% %  \paragraph{Notations and Preliminaries} For training, given batch of images $\{I_{1,...,n}\}$, we obtain a set of proposals $\bm{p}$ for the overall images via regional proposal network (RPN)~\cite{centernet2}. Among the overall proposals, we obtain positive proposals $\bm{p_{\text{pos}}}$ whose IoUs w.r.t. one ground-truth bounding box $b \in \mathcal{C}^{\text{B}} $ are higher than a threshold (i.e. 0.5).
%  %Since RPN is pre-trained on base classes as in \cite{detic}, RPN proposals can partially or fully localize base class objects.
 
%  %The positive proposals are then vectorized into one dimensional embedding $\bm{r} \in \mathbb{R^{M}}$ through detector head with ROI-Align~\cite{mask_rcnn} and cascade classification layers~\cite{cascade_rcnn}. For classification training w.r.t. base class objects, we applied cross entropy (CE) loss using cosine similarity b.t.w. regional embeddings and text embeddings of base class $\mathcal{T}(\mathcal{C}^{\text{B}})$ as in~\cite{vild}.



% %Several works \cite{} utilize additional unlabeled datasets and vocabulary of novel classes $\mathcal{C}^{\text{B}}$  to learn the representations of novel classes. However, the performance on test dataset of non-overlapped novel classes are limited. To this end, 
% %To enhance the classification ability on novel classes even without the prior knowledge of novel classes, we propose the learning strategy which train an OVOD model with proxy-novel classes which generated via class-wise mixup between representations of base classes. Overall framework of ProxyDet is illustrated in Fig \ref{fig:overview}. 
% %In the subsequent section, we describe how to synthesize proxy-novel class representations in Section \ref{method:learning_proxy_novel_classes_3_2}.
% % In the subsequent sections, we firstly describe how to synthesize proxy-novel class representations in Section \ref{method:learning_proxy_novel_classes_3_2}, followed by the enhanced methodologies for more robust and better novel class approximation in Section \ref{method:towards_better_robustness_and_novel_approximation_3_3}.

% \subsection{ProxyDet: Learning Proxy Novel Classes via Class-wise Mixup}
% \label{method:learning_proxy_novel_classes_3_2}

% % 3.2. LEARNING PROXY-NOVEL class representations BY CLASS-WISE Mixup
% %     1. mixup 
% %         1. 어떻게 mixup하는거고 (formulation. base class cross entropy설명 필요.)
% %         2. architecure flow 더 자세히 설명
% %         3. algorithm 설명 (simple하다)
% %         4. test-time fusion 설명

% % To facilitate the model's ability to recognize new categories during test phase, it is essential to learn the visual and textual representations of novel classes. Specifically, regional embedding of a novel class proposal $p^{\text{novel}}$, namely $r^{\text{novel}} = \mathcal{R}(p^{\text{novel}})$, should be closely positioned to the text embedding of the corresponding novel class $\mathcal{T}(c^{\text{novel}})$ where $c^{\text{novel}} \in \mathcal{C}^{N}$. Therefore, we train $\mathcal{R}$ by approximately regularizing the regional embedding of proxy-novel class $r^{\text{proxy}} \approx r^{\text{novel}}$ where  $c^{\text{proxy}} \in \mathcal{C}^{\text{proxy}}$, to minimize its distance with the proxy-novel text embedding $\mathcal{T}(c^{\text{proxy}}) ~\approx \mathcal{T}(c^{\text{novel}})$.
% To facilitate the model's ability to recognize new categories during test phase, it is essential to learn the visual and textual representations of novel classes. Specifically, regional embedding of a novel class proposal should be closely positioned to the text embedding of the corresponding novel class. Therefore, we train the detector by approximately regularizing the regional embedding of the proxy-novel class to minimize its distance with the proxy-novel text embedding.


%  \paragraph{Proxy Loss.} 
% % 위 목적을 달성하기 위하여, $r^{proxy}~= r^{novel}$이 proxy-novel text embedding $T~\mathcal{C}^{\text{N}}$ (which is approximately novel as show in figure 2)에 가까워지도록 학습할 수 있도록 한다. 
% Our objective can be formulated as follows:

% \begin{equation}
%     \mathcal{L}_{\text{proxy}} = \frac{1}{|\mathcal{C}^{\text{proxy}}|} \sum_{c^{\text{proxy}} \in \mathcal{C}^{\text{proxy}}} || \mathcal{T}(c^{\text{proxy}}) - r^{\text{proxy}} ||_{1}
% \label{eq:proxy_loss}
% \end{equation}

% where $T(c^{\text{proxy}})$, $r^{\text{proxy}}$ denote text embedding and regional embedding for the proxy class $c^{\text{proxy}}$, respectively.
% %$$S$ denotes number of sampling proxy-novel class from proxy-novel distribution $P_{proxy}$.
% To obtain these representations of proxy-novel class $c^{\text{proxy}}$, we present class-wise mixup between \textit{prototypical} embeddings of base classes that contain class-specific features, based on the observations from Figure \ref{fig:novel_similarity}:
% \begin{equation}
% \begin{split}
%     & \mathcal{T}(c^{\text{proxy}}) = ||\ \lambda \mathcal{T}(c^{\text{B}_{i}}) + (1 - \lambda) \mathcal{T}(c^{\text{B}_{j}})\ ||_{2} \\
%     & r^{\text{proxy}} = ||\ \lambda \bar{r}^{\text{B}_{i}} + (1 - \lambda) \bar{r}^{\text{B}_{j}}\ ||_{2}
% \end{split}
% \label{eq:mixup}
% \end{equation}

% where $\mathcal{T}(c^{\text{B}_{i}})$ and $\bar{r}^{\text{B}_{i}}$ denote the prototypical text and visual embedding of base class $c^{\text{B}_{i}} \in \mathcal{C}^{\text{B}}$, respectively. $\lambda $ is sampled from $Beta(\gamma, \gamma)$ and $c^{\text{B}_{i}}, c^{\text{B}_{j}}$ are random-uniformly sampled from one of base classes appeared within image batch. Notably, although class-specific text embeddings $\mathcal{T}(c^{\text{B}_{i}})$ can be easily obtained by forwarding through largely pretrained text encoder $\mathcal{T}$, acquiring class-specific regional embedding $\bar{r}^{\text{B}_{i}}$ is non-trivial since there are a number of candidate regional embeddings that can represent class $c^{\text{B}_{i}}$. A simple and naive solution is to estimate the centroid of all the positive regional embeddings $\bm{p^{pos}} \in c^{\text{B}_i}$ where their assigned class labels ($c$ in Eq. \ref{eq:proposal_def}) are all equal to $c^{\text{B}_{i}}$:

% \begin{equation}
% \begin{split}
%     & \bar{r}^{\text{B}_{i}} = || \sum_{r \sim \bm{r}^{\text{B}_{i}}} F(r) * r\ ||_{2}, \\
%     & F(r) = \frac{1}{|\bm{r}^{\text{B}_{i}}|}
% \end{split}
% \label{eq:prototype}
% \end{equation}

%  Notably, $\bm{r}^{\text{B}_{i}} = \{R(p^{pos}) \mid p^{pos} \in \bm{p^{pos=\text{B}_i}} \}$.
%  % refers to a set consisting of positive regional embedding $r^{pos}$ that is matched with objects that have class label $c_{\text{B}_{i}}$.
%  $F(r)$ denotes weighting function for each positive regional embedding $r$.

% % RPN에서 나온 proposal들을 class별로 groupping한다. (by IoU Thresholding) 
% % base class를 대표할 수 있는 prototype을 만든다.
%  % base prorotype들을 활용하여 proxy novel prototyep 을 만들고, 이게 proxy-novel text embedding에 가까워지도록 mixup을 통해 학습하도록 한다.
%  % mixup formulation. batch내에 있는 모든 class들에 대해서 class-wise mixup. pair결정은 random으로 표기. (equation 하나 나와야할듯.)

% % class를 대표할 수 있는 prototype embedding 구해서,
% % mixup(prototype embedding of class a, prototype embedding of class b)이 mixup(text embedding of class a, text embedding of class b)에 따라가게끔 학습한다. 

% \paragraph{Robust Prototype.} Simply averaging all the regional embeddings for constructing a prototype embedding as in Eq (\ref{eq:prototype}) can be sub-optimal since the visual semantics and contexts of the proposals that belong to the same class vary (Figure \ref{fig:prototype}). To cope with this, we propose to construct a robust prototype tailored to better represent the class specific features by modulating the weighting function $F(r)$ with proposal quality-aware measure $L$:

% \begin{equation}
% \begin{split}
%     F(r) = \frac{\text{exp}(L(r))}{\sum_{\tilde{r} \sim \bm{r}^{\text{B}_{i}}} \text{exp}( L(\tilde{r}))}
% \end{split}
% \label{eq:prototype_weighting_function}
% \end{equation}

% Notably, $L$ can be defined by \textit{objectness score} from RPN or \textit{IoU} with matched ground-truth box. Through Eq (\ref{eq:prototype_weighting_function}), our proxy-novel synthesis (Eq (\ref{eq:mixup})) is conditioned on more robust prototype embeddings that can better estimate the base class representations.

% \input{figures/prototype}

% % As the positive proposals contain different visual contexts as shown in Figure \ref{}, we propose to construct a robust prototype tailored for better representing the class-specific features. 

% % Therefore, Simply averaging all the regional embeddings $r \sim \bm{r}_{\text{B}_i}$ for constructing prototype embedding might induce 

% % For constructing the prototype of embedding $$, 

% %         1. instance-wise mixup은 기존에 있었다. 그러나, ~~이유로 robust한 prototype embedding을 못만들고 , mixup할때 sub-optimal일수있다.
% %         2. 따라서, 우리는 좀 더 robust한 prototype을 가지고 class-wise mixup를 제안한다. 
% %         3. 그러나, quality가 좋지 않은 embedding들이 prototype에 참여되면, 이또한 potential caveat이다.
% %         4. 따라서, objectness score나 iou를 기반으로 좋은 quality proposal embedding만 가지고 prototype embedding을 만들어 내겠다.

%  \paragraph{Separated Head.} Since our proxy loss Eq (\ref{eq:proxy_loss}) aims to enhance novel classification while conventional CE loss focuses on that of base classes, we applied each of loss separately on two separated detector heads with identical architecture~\cite{vild, f-vlm}. 
%  For inference, we combine both of classification scores from two heads by geometric mean, following~\cite{f-vlm}:

% \begin{equation}
%     s_i = 
% \begin{cases}
%     (r' w^{\top})^{1-\alpha}_{i} *  (r w^{\top})^{\alpha}_{i}, & \text{if } i \in \mathcal{C}^{\text{B}} \\
%     (r' w^{\top})^{1-\beta}_{i} *  (r w^{\top})^{\beta}_{i}, & \text{if } i \in \mathcal{C}^{\text{N}}
% \end{cases}
% \label{eq:score_fusion}
% \end{equation}

% where $w = \mathcal{T}(\mathcal{C}^{\text{B}} \cup \mathcal{C}^{\text{N}})$, $\ s_i$ is final classification score for $i$-th class and $r$ and $r'$ are regional embedding from a head trained with proxy loss and the other head with CE loss, respectively.  $\alpha, \beta \in [0, 1]$ determines the ratio of reflecting classification scores from proxy loss head for base/novel categories.
%  % classification loss랑 mixup loss랑 contention이 있어서,  똑같은 roi head 구조를 2개 둬서, 서로 다른 supervision이 들어가도록 했다.

%  % \paragraph{Inference}
%  % inference할때는 geometric mean해줬다 (f-vlm) 
 
% % 왜 novel class에 대해 잘 동작할 수 있는가? 1번 이유) 실제로 novel class에 대한 proposal이 조금 더 proxy-novel space에 가까워지도록 되게 되서 (which is approximately novel as show in figure 2), 더 novel class에 대한 classification을 잘할 수 있게 된다.
% % 왜 novel class에 대해 잘 동작할 수 있는가? 2번 이유) detector가 l1으로 proxy class text embedding에 유사해지도록 학습되면, 실제 novel class object가 들어왔을때, 이를 novel class text embedding에 유사해지도록 할 수 있을것이다. 따라서, novel class에 대해서 더욱 classification을 잘할 수 있게 된다.
% % dense하게 한다. 그래서 최대한 많은 novel class들을 approximate되게끔한다.

% % \subsection{Towards better robustness and novel class approximation}
% % \label{method:towards_better_robustness_and_novel_approximation_3_3}
% % \paragraph{Robust Prototype} For constructing the class-specific regional embeddings, we simply averaged regional embeddings of a class   leverage Instead of instance-wise mixup, 

% % 3.3. TOWARDS better robustness and novel class approximation
% %     1. mixup granularity
% %         1. instance-wise mixup은 기존에 있었다. 그러나, ~~이유로 robust한 prototype embedding을 못만들고 , mixup할때 sub-optimal일수있다.
% %         2. 따라서, 우리는 좀 더 robust한 prototype을 가지고 class-wise mixup를 제안한다. 
% %         3. 그러나, quality가 좋지 않은 embedding들이 prototype에 참여되면, 이또한 potential caveat이다.
% %         4. 따라서, objectness score나 iou를 기반으로 좋은 quality proposal embedding만 가지고 prototype embedding을 만들어 내겠다.
% %     2. mixup class pair.
% %             1. random하게 class를 섞는 방법
% %             2. novel class pairing: novel class를 조금 더 근사해보기 위해서, ideal case를 해본다. (using intractable knowledge: novel category space)
% %     3. distill과의 비교? (optional)
% %         1. 어떤점에서 distill과 차별성이 있는지 짚어주기. 의미론적으로.
% %             1. text embedindg 직접 맞춰준다 (which has similar semantics with novel classes)
% %             2. training time때 offline proposal들을 뽑는 공수가 안든

% % \begin{enumerate}
% %     \item \todo{ identified the limitations of existing approaches}
% %     \item \todo{ I am tackling existing solutions limitations.}
% %     \item \todo{ giving an overview of my approach, telling how it works in a general way. (explained your approach in general terms)}
% %     \item \todo{ motivated your solution using Figure: show a picture of how your approach will deal with such a problem. }
% % \end{enumerate}



==> tables/table2_3_merged.tex <==
\begin{table*}[t]
    \begin{minipage}[b]{0.42\linewidth}
        \input{tables/table2_ov_lvis}
    \end{minipage}
    \hfill 
    \begin{minipage}[b]{0.42\linewidth}
        \input{tables/table3_ov_coco}
    \end{minipage}
\end{table*}
